Ordered Memory

Stack-augmented recurrent neural networks (RNNs) have been of interest to the deep learning community for some time. However, the difficulty of training memory models remains a problem obstructing the widespread use of such models. In this paper, we propose the Ordered Memory architecture. Inspired by Ordered Neurons (Shen et al., 2018), we introduce a new attention-based mechanism and use its cumulative probability to control the writing and erasing operation of the memory. We also introduce a new Gated Recursive Cell to compose lower-level representations into higher-level representation. We demonstrate that our model achieves strong performance on the logical inference task (Bowman et al., 2015)and the ListOps (Nangia and Bowman, 2018) task. We can also interpret the model to retrieve the induced tree structure, and find that these induced structures align with the ground truth. Finally, we evaluate our model on the Stanford SentimentTreebank tasks (Socher et al., 2013), and find that it performs comparatively with the state-of-the-art methods in the literature.

==> intro-old.tex <==

\section{Introduction}

\citet{fodor1988connectionism} claim that ``cognitive capacities always exhibit certain symmetries, so that the ability to entertain a given thought implies the ability to entertain thoughts with semantically related contents," and use the term \emph{systematicity} to describe this phenomenon.
While loosely defined, more recent empirical studies  have shown that knowing the right structure when composing lower level symbols to form a representation of the expression can give rise to systematic generalisation \citep{bowman2015tree,bahdanau2018systematic}.

Exploiting known symmetries in the structure of the data has been a useful technique for achieving good generalisation capabilities in deep learning, particularly in the form of convolutions \citep{fukushima1980neocognitron}, which leverages parameter-sharing.
%This is done by parameter-sharing that results in an equivariant transformation of the input data.
If we consider architectures  used in \citet{socher2013recursive} or \citet{tai2015improved}, the same recursive operation is performed at known points along the input where the substructures are meant to be composed. 
%If we compare this to recurrent neural networks (RNNs), a function is used repeatedly to compose the previous hidden state with the current input, but this method of composition results in a left-branching tree structure that may not be suitable for most tasks.
\citet{lake2017generalization} explores RNNs and their capacity for systematic generalisation (or lack thereof.)
%So we know structure exists in language, and parameter-sharing is used in the case of RNNs, but the structure is wrong.




In \citet{shen2018ordered}, the authors introduce an inductive prior in the form of the Ordered Neurons (ON-LSTM) architecture that relates to the tree-structured form of grammars.
However, the model is not restricted to learn the same composition function at every level of the tree it induces. (Use example to make this point clearer)
While they demonstrate the capability of the model to induce parse trees for sentences, the model does so \emph{in spite of} rather than \emph{because of} the given architecture.

In this paper, we propose a model architecture, the Ordered Memory (OM), that tries to overcome these issues with RNNs by applying the composition function over a learned structure of the input.
We demonstrate that this method of composition generalises to some tasks where the ON-LSTM does not, while still retaining the same interpretability of the ON-LSTM.

% If we assume that normal RNNs when applied to such tasks implicitly do some form of parsing, they have two challenges that the learning procedure needs to overcome: a) the hidden state has to maintain the representation of a partial sub-tree as it is reading the input sentence sequentially, and b) it performs all operations a fixed transformation function from one timestep to the next, with no structure imposed (aside from the fact that it is usually a linear transform)

%Ideally, when composing constituents, the model should perform the composition using the same function, regardless of where the constituents are represented in the hidden state.
%In other words, constituent composition should be equivariant to the location of the representations in the hidden state.
% However, in order to demonstrate this, models with full knowledge of the compositional structure of the input are compared to more general architectures that take in sequential input, like an recurrent neural network (RNN).
%However, using these compositional structures, even when they are available, makes it difficult to scale as each instance of the dataset requires a different structure, removing the efficiency which minibatch training gives deep learning.
%Moreover, the true compositional structure is almost never available.
%Some approaches attempt to learn the structure from data in an unsupervised manner \citep{shen2017neural,jacob2018learning}.










% MNLI Results
\subsection{Natural Language Inference}
\citet{williams2017broad} is a natural language logical inference tasks that require the model to discern the logical relationships between pairs of sentences.
The possible classes are \texttt{entailment}, \texttt{contradiction} and \texttt{neutral}.

\textcolor{red}{Need to update once experiments are done.}
%\begin{table}[]
%\small
%    \centering
%    \begin{tabular}{l c c c}
%    \toprule
%            & SNLI & Matched & Mismatched \\
%     Method & (\%) & (\%) &  (\%) \\
%    \midrule
%        \citet{radford2018improving} &  89.9 & 82.1 & 81.4 \\
%        \citet{yoon2018dynamic} &  87.4  & -- & -- \\
%    \midrule
%        Ours (GloVe)                &  & \\
%        Ours (ELMo)                 &   & \\
%    \bottomrule
%    \end{tabular}
%    \caption{Accuracy on the SNLI and MultiNLI tasks in both Matched and %Mismatched settings.}
%    \label{tab:nli}
%\end{table}

\begin{table}
\setlength{\tabcolsep}{3.5pt} % Default value: 6pt
\small
\begin{center}
\begin{tabular}{l cc }
\toprule
Model & Acc. \\
\midrule
LSTM\(\dagger\) & 69.1 \\
SPINN\(\dagger\) & 67.5 \\
RL-SPINN\(\dagger\) & 67.4 \\
Gumbel Tree-LSTM\(\dagger\) & 69.5 \\
\citet{havrylov2019cooperative} & 70.7$\pm$0.3\\
%\midrule
%\citet{radford2018improving} & 82.1 \\
\midrule
Ours & 71.1 (ongoing) \\
\bottomrule
\end{tabular}
\end{center}
\caption{Results on MultiNLI. \(\dagger\): results are taken from \citet{williams2018latent}.}
\label{table:mnli}
\end{table}

